Spatiotemporal Pattern Recognition in Single Mixed-Signal VLSI Neurons with Heterogeneous Dynamic Synapses

Mixed-signal neuromorphic processors with brain-like organization and device physics offer an ultra-low-power alternative to the unsustainable developments of conventional deep learning and computing. However, realizing the potential of such neuromorphic hardware requires efficient use of its heterogeneous, analog neurosynaptic circuitry with neurocomputational methods for sparse, spike-timing-based encoding and processing. Here, we investigate the use of balanced excitatory-inhibitory disynaptic lateral connections as a resource-efficient mechanism for implementing a thalamocortically inspired Spatiotemporal Correlator (STC) neural network without using dedicated delay mechanisms. We present hardware-in-the-loop experiments with a DYNAP-SE neuromorphic processor, in which receptive fields of heterogeneous coincidence-detection neurons in an STC network with four lateral afferent connections per column were mapped by random input-sampling. Furthermore, we demonstrate how such a neuron was tuned to detect a particular spatiotemporal feature by discrete address-reprogramming of the analog synaptic circuits. The energy dissipation of the disynaptic connections is one order of magnitude lower per lateral connection (0.65 nJ vs 9.6 nJ per spike) than in the former delay-based hardware implementation of the STC.

==> notes.tex <==
% doi: 10.3389/fnins.2021.651141
% approach is the notion that replacing the abstract neuron used in most deep networks with a more biologically- plausible spiking neuron might lead to savings in both energy and resource cost
% rate-coded spiking network implementations will not be more energy or resource efficient than the original ANN, concluding that more imaginative uses of spikes are required to displace conventional ANNs as the dominant computing framework for neural computation
% Such approaches do exist and we wish to encourage others to adopt the same mindset. A group of researchers at TU Graz demonstrated an image recognition network in which each neuron produces at most one spike (Stöckl and Maass, 2021), while also proposing another distinct encoding using two spikes per neuron (Stöckl and Maass, 2020). Very sparse codes have been demonstrated as more energy efficient than equivalent ANN networks, even with spike rates as low as 0.24 spikes per neuron to perform an inference (Lee et al., 2019; Wu J. et al., 2019; Wu Y. et al., 2019). FPGA-based circuits using very sparse encoding combine good accuracy with low power when applied to classification tasks (Mostafa et al., 2017). Another slightly older line of enquiry is the use of rank-order coding, a form of temporal encoding that may be relevant to understanding how the retina encodes information (Thorpe and Gautrais, 1998; Furber et al., 2007; Portelli et al., 2016).
% These examples illustrate that more efficient encoding methodologies are readily achievable. They have the potential to avoid the inefficiencies we have outlined in the implementation of rate-coded networks. The path towards truly mould-breaking neurally-inspired computation for artificial systems should focus on information encoding as the way forward.
%
% doi:10.1038/nn.4243
% Recent years have seen a growing interest in inhibitory interneurons and their circuits. A striking property of cortical inhibition is how tightly it balances excitation. Inhibitory currents not only match excitatory currents on average, but track them on a millisecond time scale, whether they are caused by external stimuli or spontaneous fluctuations. We review, together with experimental evidence, recent theoretical approaches that investigate the advantages of such tight balance for coding and computation. These studies suggest a possible revision of the dominant view that neurons represent information with firing rates corrupted by Poisson noise. Instead, tight excitatory/inhibitory balance may be a signature of a highly cooperative code, orders of magnitude more precise than a Poisson rate code. Moreover, tight balance may provide a template that allows cortical neurons to construct high-dimensional population codes and learn complex functions of their inputs.

% Spike-time code
%Spike-time based neural code...\cite{sheik2017spike-based, guo2021neural}.

%Processing with few spikes... \cite{rullen1998face, stockl2021optimized}.
%...\cite{davidson2021comparison}.

%Coincidence detection... \cite{risi2020stereo}.

%Receptive fields... \cite{baruzzi2020gabor-like}.

%Dendritic pattern detection... \cite{leugering2020event-based}.

%Efficient Balanced Networks... \cite{deneve2016efficient}.

%DYNAP-SE energy estimation \cite{bauer2019real-time}

%Adaptive Extreme Edge Computing for Wearable Devices (Covi, 2021)...

%Misc...\cite{baumgartner2020visual}
